A cost-based multi-layer network approach for the discovery of patient phenotypes

Clinical records frequently include assessments of the characteristics of patients, which may include the completion of various questionnaires. These questionnaires provide a variety of perspectives on a patient's current state of well-being. Not only is it critical to capture the heterogeneity given by these perspectives, but there is also a growing demand for developing cost-effective technologies for clinical phenotyping. Filling out many questionnaires may be a strain for the patients and therefore costly. In this work, we propose COBALT -- a cost-based layer selector model for detecting phenotypes using a community detection approach. Our goal is to minimize the number of features used to build these phenotypes while preserving its quality. We test our model using questionnaire data from chronic tinnitus patients and represent the data in a multi-layer network structure. The model is then evaluated by predicting post-treatment data using baseline features (age, gender, and pre-treatment data) as well as the identified phenotypes as a feature. For some post-treatment variables, predictors using phenotypes from COBALT as features outperformed those using phenotypes detected by traditional clustering methods. Moreover, using phenotype data to predict post-treatment data proved beneficial in comparison with predictors that were solely trained with baseline features.

==> algo1_withQ.tex <==
\begin{algorithm}
\caption{
\textbf{\COBALT{} Initialization:}
%\textbf{Initial Solution}: 
Pseudo code for choosing the first layer}
\label{start_solution}
\begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \Require $G$
 \Ensure $g_{bestsingle}$  
   \State $\mathcal{S}_{single}, Q \gets \{ \emptyset, \emptyset\}$

%   \State $\mathcal{S}, Q, N \gets \{ \emptyset, \emptyset, \emptyset \}$
  \For {$g \in G$}
    %\State $n_{incumbent} \gets g$
  \State $(S_{inc}, q_{inc}) \gets  Leiden(g)$\par
  \State add $S_{inc}$ to $\mathcal{S}_{single}$ and $q_{inc}$ to $Q$ %\par\hskip\algorithmicindent and $n_{inc}$ to $N_{all}$\par
  \EndFor
  \State $g_{bestsingle} \gets$ $g$ with $\max(Q)$\\
  \Return $g_{bestsingle}, \mathcal{S}_{single}$

% \Return $g_{bestsingle}, S_{single}, N_{all}$
\end{algorithmic}
\end{algorithm}
% explain the algorithm

The input of this algorithm is the set of all single-layer graphs $G$. 
%that is constituted by one graph per layer. 
For each $g\in{}G$, \COBALT{} invokes the Leiden algorithm 
%is executed and 
which builds a set of communities and returns two objects:
%are discovered. The outputs are of two types: 
the partition $S_{inc}$, which encompasses the community membership of each node for the incumbent graph $g \in G$, and $q_{inc}$ -- the modularity of 
%the incumbent partition 
$S_{inc}$. The graph with the best modularity ($g_{bestsingle}$) is chosen as returned as initial solution of \COBALT{}.
%and it forms the output of the algorithm.

==> algo2_orig.tex <==
\begin{algorithm}
\caption{
Iterative Layer Selection: Pseudo-code of the subsequent iterations of \COBALT{}
%\textbf{Layer Selection}: Pseudo code of the search algorithm
}
\label{global_search}
\begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
%  \Require $G, g_{bestsingle}, S_{single}, N_{all}$
 \Require $G, g_{bestsingle}, \mathcal{S}_{single}$

 \Ensure $s_{best}$ (best solution)
  \State $G_{candidates} \gets G \backslash \{g_{bestsingle}\}$
  \State $s_{inc} \gets S \in S_{single}$ that corresponds to $g_{bestsingle}$
  \State $\mathcal{L} \gets g_{bestsingle}$ 
%   \State $n_{inc} \gets n \in N_{all}$ that corresponds to $g_{bestsingle}$
  \While{$G_{candidates} \neq \emptyset$ and \textit{SC1} False}
     \State $g_{inc} \gets \argmin_{u\in G_{candidates}} cost(S_u,S_{inc})$
    % \For{$g \in G_{candidates}$}
    %     \State $s_g \gets s \in S_{single}$ that corresponds to $g$
    %     \State $cost_{inc, g}\gets$\textit{cost} $(s_{inc}, s_g)$
    % \EndFor
    % \State $g_i\gets g \in G_{candidates}$ with $min(cost)$
    \State $\mathcal{L} \gets$ add the layer $g_{inc}$ to $\mathcal{L}$
    %\State $n_{test} \gets$ add a layer $g_i$ to $n_{inc}$
    \State $s_{inc}, q_{inc} \gets Leiden(\mathcal{L})$ 
    %\State $s_{test}, q_{test}, n_{test} \gets Leiden(n_{test})$ 
%   \If{$q_{test} > q_{inc}$}
%     \State $s_{inc} \gets s_{test}$
%     \State $q_{inc} \gets q_{test}$
%     \State $n_{inc} \gets n_{candidate}$
%   \EndIf
   \State  $G_{candidates} \gets G_{candidates} \backslash \{g_{inc}\}$
  \EndWhile
  \State $s_{final} \gets s_{inc}$\\
 \Return $s_{final}$
\end{algorithmic} 
\end{algorithm}

The input of Algorithm \ref{global_search} is the set of graphs $G$ and the outputs of Algorithm \ref{start_solution}. $g_{bestsingle}$ is the first graph, which represents the first layer of the MLN structure to be built.
$\mathcal{L}$ denotes the single- or multi-layer structure of the incumbent iteration. More specifically, this variable is equivalent to $g_{bestsingle}$ in the initial phase of algorithm, but as layers are added, $\mathcal{L}$ is updated to a multi-layer network structure.

To decide which further layers should be added, a list of candidates $G_{candidates}$ is created and dynamically updated to include only graphs that were not added yet to $\mathcal{L}$. No repeated layers can be added and therefore $G_{candidates}$ should be empty at the last iteration of the algorithm. 
We consider the start of Algorithm \ref{global_search} as iteration 2, since the iteration 1 represents Algorithm \ref{start_solution}. The number of iterations is equal to the number of layers. 

Therefore, at the beginning of the algorithm $g_{bestsingle}$ is removed from the set of graphs $G$ and this results into the set of candidates $G_{candidates}$. Then, the layer cost is computed for all candidates $u \in G_{candidates}$. This computation is made between the pair $g$ and $\mathcal{L}$, in which $g$ will change according to the candidate that is being tested. The cost is computed based on the community similarity between both layers and the availability ratio term. Hence, the community memberships are required as inputs: $S_u$ for the candidate and $S_{inc}$ for the incumbent partition. The candidate with the lowest cost, $g_{inc}$, is selected and added to $\mathcal{L}$. This consists in the first MLN (a 2-layer network). Modularity of this incumbent solution, $q_{inc}$, is computed. The subsequent iterations follow to the same premise. The algorithm runs while there are candidates in $G_{candidates}$ and while \textit{SC1} is not True. We define \textit{SC1} in the next subsection (see subsection \ref{stopping_criterion_methodology}).

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.

\bibitem[Puga2021]{C. Puga, U. Niemann, V. Unnikrishnan, M. Schleicher, W. Schlee, and M. Spiliopoulou, “Discovery of Patient Phenotypes through Multi-layer Network Analysis on the Example of Tinnitus,” 2021 IEEE 8th Int. Conf. Data Sci. Adv. Anal., pp. 1–10, 2021, doi: 10.1109/dsaa53316.2021.9564158.}

\bibitem[Brodka2018]{P. Bródka, A. Chmiel, M. Magnani, and G. Ragozini, “Quantifying layer similarity in multiplex networks: A systematic study,” R. Soc. Open Sci., vol. 5, no. 8, 2018, doi: 10.1098/rsos.171747.}

\bibitem[Tantardini2019]{M. Tantardini, F. Ieva, L. Tajoli, and C. Piccardi, “Comparing methods for comparing networks,” Sci. Rep., vol. 9, no. 1, pp. 1–19, 2019, doi: 10.1038/s41598-019-53708-y.}
\end{thebibliography}

\bibitem[Ghawi2022]{R. Ghawi and J. Pfeffer, “A community matching based approach to measuring layer similarity in multilayer networks,” Soc. Networks, vol. 68, no. April 2021, pp. 1–14, 2022, doi: 10.1016/j.socnet.2021.04.004.}

\bibitem[tbf12]{K. V. Greimel, M. Leibetseder, J. Unterrainer, and K. Al-begger,  “Ist  Tinnitus  meßbar?  Methoden  zur  Erfassungtinnitusspezifischer Beeintr ̈achtigungen und Pr ̈asentationdes  Tinnitus-Beeintr ̈achtigungs-Fragebogens  (TBF-12),”HNO, vol. 47, no. 3, pp. 196–201, 1999.}

\bibitem[mdi]{P.   Bech,   N.-A.   Rasmussen,   L.   Olsen,   V.   Noerholm,and  W.  Abildgaard,  “The  sensitivity  and  specificity  ofthe  major  depression  inventory,  using  the  present  stateexamination as the index of diagnostic validity,”Journalof  Affective  Disorders,  vol.  66,  no.  2-3,  pp.  159–164,2001.}

\bibitem[tfi]{M.  B.  Meikle,  J.  A.  Henry,  S.  E.  Griestet  al.,  “Thetinnitus functional index,”Ear & Hearing, vol. 33, no. 2,pp. 153–176, 2012.}

\bibitem[thi]{A.   McCombe,   D.   Baguley,   R.   Coles,   L.   McKenna,C. McKinney, and P. Windle-Taylor, “Guidelines for thegrading  of  tinnitus  severity:  the  results  of  a  workinggroup  commissioned  by  the  british  association  of  oto-laryngologists,  head  and  neck  surgeons,  1999,”ClinicalOtolaryngology  and  Allied  Sciences,  vol.  26,  no.  5,  pp.388–393, 2001.}

\bibitem[tq]{G.  Goebel  and  W.  Hiller,  “Tinnitus-Fragebogen  (TP)-Handanweisung,”Hogrefe, G ̈ottingen, 1998.}

\bibitem[dinati]{N. Dianati, “Unwinding the hairball graph: Pruning algorithms for weighted complex networks,” Phys. Rev. E, vol. 93, no. 1, 2016, doi: 10.1103/PhysRevE.93.012304.}

\bibitem[fruchterman]{Fruchterman, T. M., & Reingold, E. M. (1991). Graph drawing by force‐directed placement. Software: Practice and experience, 21(11), 1129-1164.}

\bibitem[kmeans]{Hartigan, J. A. and Wong, M. A. (1979). Algorithm AS 136: A K-means clustering algorithm. Applied Statistics, 28, 100–108. doi: 10.2307/2346830.}

\bibitem[agglo]{Day, William HE, and Herbert Edelsbrunner. "Efficient algorithms for agglomerative hierarchical clustering methods." Journal of classification 1.1 (1984): 7-24}

\bibitem[birch]{Zhang, Tian, Raghu Ramakrishnan, and Miron Livny. "BIRCH: an efficient data clustering method for very large databases." ACM sigmod record 25.2 (1996): 103-114.}

\bibitem[gmm1]{Biernacki, Christophe, Gilles Celeux, and Gérard Govaert. "Assessing a mixture model for clustering with the integrated completed likelihood." IEEE transactions on pattern analysis and machine intelligence 22.7 (2000): 719-725.}

\bibitem[gmm2]{Dempster, Arthur P., Nan M. Laird, and Donald B. Rubin. "Maximum likelihood from incomplete data via the EM algorithm." Journal of the Royal Statistical Society: Series B (Methodological) 39.1 (1977): 1-22.}

\bibitem[hdbscan]{Campello, Ricardo JGB, et al. "Hierarchical density estimates for data clustering, visualization, and outlier detection." ACM Transactions on Knowledge Discovery from Data (TKDD) 10.1 (2015): 1-51.}

\bibitem[optics]{Ankerst, Mihael, et al. "OPTICS: Ordering points to identify the clustering structure." ACM Sigmod record 28.2 (1999): 49-60.}

\bibitem[Rolstad2011]{S. Rolstad, J. Adler, and A. Rydén, “Response burden and questionnaire length: Is shorter better? A review and meta-analysis,” Value Heal., vol. 14, no. 8, pp. 1101–1108, 2011, doi: 10.1016/j.jval.2011.06.003.}

\bibitem[Huang2020]{X. Huang, D. Chen, T. Ren, and D. Wang, A survey of community detection methods in multilayer networks. Springer US, 2020.}

\bibitem[Ali2019]{H. T. Ali, S. Liu, Y. Yilmaz, R. Couillet, I. Rajapakse, and A. Hero, “Latent Heterogeneous Multilayer Community Detection,” in ICASSP 2019 - 2019 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP), May 2019, pp. 8142–8146, doi: 10.1109/ICASSP.2019.8683574.}

\bibitem[lucas2011]{I.   S.   Jutla,   L.   G.   Jeub,   P.   J.   Muchaet   al.,   “Ageneralized  Louvain  method  for  community  detectionimplementedinMATLAB.”[Online].Available:https://github.com/GenLouvain/GenLouvain (2011-2019)}

\bibitem[Pan2018]{Z. Pan, G. Hu, and D. Li, “Detecting communities from multilayer networks,” in Proceedings of the International Conference on Intelligent Science and Technology - ICIST ’18, 2018, pp. 6–11, doi: 10.1145/3233740.3233742.}

\bibitem[Gao2019]{X. Gao, Q. Zheng, F. A. N. Verri, R. D. Rodrigues, and L. Zhao, “Particle Competition for Multilayer Network Community Detection,” in Proceedings of the 2019 11th International Conference on Machine Learning and Computing - ICMLC ’19, 2019, vol. Part F1481, pp. 75–80, doi: 10.1145/3318299.3318320.}

\bibitem[Alimadadi2019]{F. Alimadadi, E. Khadangi, and A. Bagheri, “Community detection in facebook activity networks and presenting a new multilayer label propagation algorithm for community detection,” Int. J. Mod. Phys. B, vol. 33, no. 10, p. 1950089, Apr. 2019, doi: 10.1142/S0217979219500899.}

\bibitem[DeMeo2011]{P. De Meo, E. Ferrara, G. Fiumara, and A. Provetti, “Generalized Louvain method for community detection in large networks,” in 2011 11th International Conference on Intelligent Systems Design and Applications, Nov. 2011, no. August, pp. 88–93, doi: 10.1109/ISDA.2011.6121636.}

\bibitem[Traag2019]{V. A. Traag, L. Waltman, and N. J. van Eck, “From Louvain to Leiden: guaranteeing well-connected communities,” Sci. Rep., vol. 9, no. 1, pp. 1–12, 2019, doi: 10.1038/s41598-019-41695-z.}

\bibitem[Huang2019]{Y. Huang, A. Panahi, H. Krim, and L. Dai, “Community Detection and Improved Detectability in Multiplex Networks,” arXiv, vol. 7, no. 3, pp. 1697–1709, 2019.}

\bibitem[Weir2020]{W. H. Weir, B. Walker, L. Zdeborová, and P. J. Mucha, “Multilayer Modularity Belief Propagation to Assess Detectability of Community Structure,” SIAM J. Math. Data Sci., vol. 2, no. 3, pp. 872–900, 2020, doi: 10.1137/19m1279812.}

\bibitem[Mucha2010]{P. J. Mucha, T. Richardson, K. Macon, M. A. Porter, and J. P. Onnela, “Community structure in time-dependent, multiscale, and multiplex networks,” Science (80-. )., vol. 328, no. 5980, pp. 876–878, 2010, doi: 10.1126/science.1184819.}

\bibitem[Interdonato2020]{R. Interdonato, M. Magnani, D. Perna, A. Tagarelli, and D. Vega, “Multilayer network simplification: Approaches, models and methods,” arXiv, no. May, 2020.}

\bibitem[Dinati2016]{N. Dianati, “Unwinding the hairball graph: Pruning algorithms for weighted complex networks,” Phys. Rev. E, vol. 93, no. 1, 2016, doi: 10.1103/PhysRevE.93.012304.}

\bibitem[Subphenotypes]{E. Genitsaridi, D. J. Hoare, T. Kypraios, and D. A. Hall, “A review and a framework of variables for defining and characterizing tinnitus subphenotypes,” Brain Sci., vol. 10, no. 12, pp. 1–21, 2020, doi: 10.3390/brainsci10120938.}

\bibitem[Richesson]{R. L. Richesson, J. Sun, J. Pathak, A. N. Kho, and J. C. Denny, “A survey of clinical phenotyping in selected national networks: demonstrating the need for high-throughput, portable, and computational methods,” Artif. Intell. Med., vol. 71, pp. 57–61, 2016, doi: 10.1016/j.artmed.2016.05.005.}

\bibitem[genes]{S. Amanat, T. Requena, and J. A. Lopez-Escamez, “A systematic review of extreme phenotype strategies to search for rare variants in genetic studies of complex disorders,” Genes (Basel)., vol. 11, no. 9, pp. 1–15, 2020, doi: 10.3390/genes11090987.}

\bibitem[Huckvale2019]{K. Huckvale, S. Venkatesh, and H. Christensen, “Toward clinical digital phenotyping: a timely opportunity to consider purpose, quality, and safety,” npj Digit. Med., vol. 2, no. 1, 2019, doi: 10.1038/s41746-019-0166-1.}

\bibitem[Liang2019]{Y. Liang, X. Zheng, and D. D. Zeng, “A survey on big data-driven digital phenotyping of mental health,” Inf. Fusion, vol. 52, no. July 2018, pp. 290–307, 2019, doi: 10.1016/j.inffus.2019.04.001.}


\bibitem[Lee2020]{B. Lee, S. Zhang, A. Poleksic, and L. Xie, “Heterogeneous Multi-Layered Network Model for Omics Data Integration and Analysis,” vol. 10, no. January, pp. 1–11, 2020, doi: 10.3389/fgene.2019.01381.}

\bibitem[Kramer2020]{J. Kramer, L. Boone, T. Clifford, J. Bruce, and J. Matta, “Analysis of Medical Data Using Community Detection on Inferred Networks,” IEEE J. Biomed. Heal. Informatics, vol. 24, no. 11, pp. 3136–3143, 2020, doi: 10.1109/JBHI.2020.3003827.}

\bibitem[Yang2021]{D. Yang, Y. Jin, X. He, A. Dong, J. Wang, and R. Wu, “Inferring multilayer interactome networks shaping phenotypic plasticity and evolution,” Nat. Commun., pp. 1–17, 2021, doi: 10.1038/s41467-021-25086-5.}

\bibitem[Eggermont2004]{J. J. Eggermont and L. E. Roberts, “The neuroscience of tinnitus,” Trends Neurosci., vol. 27, no. 11, pp. 676–682, 2004, doi: 10.1016/j.tins.2004.08.010.}

\bibitem[Cima2014]{Rilana F.F. Cima, Gerhard Andersson, Caroline J. Schmidt, & James A. Henry (2014). Cognitive-Behavioral Treatments for Tinnitus: A Review of the Literature. Journal of the American Academy of Audiology, 25(01), 029–061.}

\bibitem[Cima2012]{Rilana FF Cima, Iris H Maes, Manuela A Joore, Dyon JWM Scheyen, Amr El Refaie, David M Baguley, Lucien JC Anteunis, Gerard JP van Breukelen, & Johan WS Vlaeyen (2012). Specialised treatment based on cognitive behaviour therapy versus usual care for tinnitus: a randomised controlled trial. The Lancet, 379(9830), 1951–1959.
}

\bibitem[Schlee2021]{W. Schlee et al., “Using Big Data to Develop a Clinical Decision Support System for Tinnitus Treatment,” in Choice Reviews Online, vol. 47, no. 10, 2021, pp. 175–189.}

\bibitem[Niemann2020phenotypes]{U. Niemann et al., “Phenotyping chronic tinnitus patients using self-report questionnaire data: cluster analysis and visual comparison,” Sci. Rep., vol. 10, no. 1, pp. 1–10, 2020, doi: 10.1038/s41598-020-73402-8.}

==> subsection_evaluation.tex <==
\subsection{Evaluation}\label{subsection_evaluation}
In the context of the current application, ground-truth is not available and hence we conduct more than one type of evaluation. Despite the fact that we aim to achieve the objective proposed in Equation \ref{max_quality}, this objective only focus on the quality partition with respect to the network properties and not the domain in which it is applied. This type of evaluation is independent on the type of network data we use and it is transferable to other domains, i.e., it is not restricted to the medical data. 

Within the scope of our application, however, we want to examine how well the algorithm performs in the domain in which it is tested.
We do this by training a regressor to predict the post-treatment data (at $t_1$), per questionnaire, using as features the age, gender, score of that questionnaire at admission (at $t_0$) and the community to which each patient (node) is assigned to.
We test this for all iterations - the regressor is trained for all community partitions generated.

Besides, we test it across all questionnaires (target variables). For example, in iteration 1 we only have a single-layer network but since the nodes represent the patients, we may have information about their scores in another questionnaires. Therefore, we can train a regressor of the partition from iteration 1 using as the target variable of our regressor another questionnaire and study how transferable are the communities found with the one questionnaire.

To summarize, we train one regressor per pair (target; iteration).
The regressor models used are: linear regressor, ridge, LASSO and SVR (support vector regressor). A grid search to the hyperparameters of these models is conducted with 10-fold cross validation. The error metrics used are: MAE (mean absolute error), MSE (mean squared error) and $R^2$.

Lastly, we compare our algorithm with traditional clustering algorithms. The algorithms are not directly comparable, but the type of evaluation aforementioned makes it possible to compare them. The same logic is employed: a regressor is trained per clustering solution and the prediction errors of post-treatment data are compared. 
The clustering models takes all the questionnaire scores as features, while our community detection algorithm only uses the data from all features when it gets to the last iteration. Hence, this should be taken into account when interpreting the results.

Another contrast between clustering models and our proposed algorithm is that clustering models do not handle missing values, whereby only data without missing values is used to train these models. The clustering techniques used are: (i) agglomerative hierarchical clustering \cite{agglo}; (ii) BIRCH \cite{birch}, (iii) Gaussian Mixture Models with the Expectation Maximization algorithm \cite{gmm1, gmm2}, (iv) HDBSCAN \cite{hdbscan}, (v) k-means \cite{kmeans} and (vi) OPTICS \cite{optics}. 
